Corpus Distillation for Effective Fuzzing: A Comparative Evaluation

Mutation-based fuzzing typically uses an initial set of non-crashing seed inputs (a corpus) from which to generate new inputs by mutation. A corpus of potential seeds will often contain thousands of similar inputs. This lack of diversity can lead to wasted fuzzing effort by exhaustive mutation from all available seeds. To address this, fuzzers come with distillation tools (e.g., afl-cmin) that select the smallest subset of seeds that triggers the same range of instrumentation data points as the full corpus. Common practice suggests that minimizing the number and cumulative size of the seeds leads to more efficient fuzzing, which we explore systematically. We present results of 34+ CPU-years of fuzzing with five distillation approaches to understand their impact in finding bugs in real-world software. We evaluate a number of techniques, includibng the existing afl-cmin and Minset, and also MoonLight---a freely available, configurable, state-of-the-art, open-source, tool. Our experiments compare the effectiveness of distillation approaches, targeting the Google Fuzzer Test Suite and a diverse set of six real-world libraries and programs, covering 13 different input file formats across 16 programs. Our results show that distillation is a necessary precursor to any fuzzing campaign when starting with a large initial corpus. We compare the effectiveness of alternative distillation approaches. Notably, our experiments reveal that state-of-the-art distillation tools (such as MoonLight and Minset) do not exclusively find all of the 33 bugs (in the real-world targets) exposed by our combined campaign: each technique appears to have its own strengths. We find (and report) new bugs with MoonLight that are not found by Minset, and vice versa. Moreover, afl-cmin fails to reveal many of these bugs. Of the 33 bugs revealed in our campaign, seven new bugs have received CVEs.

==> approach-figs.tex <==
\begin{figure}[h]
  \centering
  \setlength{\lineskip}{1.5ex}% increase spacing
  \begin{subfigure}[b]{0.6\linewidth}
    \centering
    \scalebox{0.5}{
      \begin{tikzpicture}
        \example[1]
      \end{tikzpicture}
    }
    \caption{Coverage matrix}\label{fig:WorkingExampleMain}
  \end{subfigure}
  \begin{subfigure}[b]{0.49\linewidth}
    \centering
    \scalebox{0.5}{
      \begin{tikzpicture}
        % Singularity
        \example[0]
        \block[green]{1}{6} \block[green]{2}{6} \block[green]{3}{6}
        \block[green]{4}{6} \block[green]{5}{6}
      \end{tikzpicture}
    }
    \caption{Singularity}\label{fig:SingularityMain}
  \end{subfigure}
  \begin{subfigure}[b]{0.49\linewidth}
    \centering
    \scalebox{0.5}{
      \begin{tikzpicture}
        % Exotic
        \example[0]
        \block[cyan]{1}{2} \block[cyan]{1}{3} \block[cyan]{1}{5}
        \block[cyan]{1}{7}
        \highlight{1}{3} %mark the exotic seed-block
      \end{tikzpicture}
    }
    \caption{Exotic row}\label{fig:ExoticMain}
  \end{subfigure}
  \begin{subfigure}[b]{0.49\linewidth}
    \centering
    \scalebox{0.5}{
      \begin{tikzpicture}
        % Row Domination
        \example[0]
        \block[red]{5}{1} \block[red]{5}{2} \block[red]{5}{4}
        \block[red]{5}{5}
        \block[red]{5}{7}
        % 
        \block[yellow]{2}{2} \block[yellow]{2}{7}
        \block[yellow]{3}{1} \block[yellow]{3}{4} \block[yellow]{3}{5}
        \block[yellow]{4}{2} \block[yellow]{4}{5} \block[yellow]{4}{7}
      \end{tikzpicture}
    }
    \caption{Row dominance}\label{fig:RowDominanceMain}
  \end{subfigure}
  \begin{subfigure}[b]{0.49\linewidth}
    \centering
    \scalebox{0.5}{
      \begin{tikzpicture}
        % Column Domination
        \example[0]
        \block[red]{1}{5} \block[red]{3}{5} \block[red]{4}{5}
        \block[red]{5}{5}
        % 
        \block[yellow]{3}{1} \block[yellow]{5}{1}
        \block[yellow]{1}{3}
        \block[yellow]{3}{4} \block[yellow]{5}{4}
      \end{tikzpicture}
    }
    \caption{Column dominance}\label{fig:ColumnDominanceMain}
  \end{subfigure}
  \caption{Coverage minimization examples.  Rows $s_i$ represent seeds;
    columns $e_i$ represent all possible edges.  In (a), gray elements indicate edges
    that are covered by a given seed, while white elements indicate those
    edges that are uncovered.}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "moonlight"
%%% End:


==> section-approach.tex <==
\section{Our Approach}\label{sec:Approach}

We now provide an intuitive description of our corpus distillation
algorithm.
% A more detailed presentation of the theory, key accompanying proofs,
% and implementation appear in \cref{sec:Theory-Appendix}.

\subsection{Problem Definition}

Recall that our fundamental task is \emph{distillation}: the removal
of members of a set of seeds (a \emph{corpus}) while retaining the
\emph{coverage} of the corpus.  A target program (or library) has a
finite set of edges between its constituent basic blocks, and any
given seed will cause a subset of these edges to be traversed when the
target is executed on that seed.  This seed's set of edges is its
\emph{coverage}, and the coverage of a corpus is the union of the
coverages of each of its seeds.

Following current state-of-the-art fuzzers (in particular, AFL), we
make the assumption that edge coverage is a good approximation of
target behavior, and thus: fuzzing over a distilled corpus will
discover as many bugs as fuzzing over the original corpus.  To the
extent that this assumption is not true, we are willing to forgo lost
behaviors (which may lead to bugs) in exchange for increased testing
speed in the fuzzing process.  Pragmatically, we hope that this
increased speed will result in the discovery of more bugs.
Empirically, this hope is indeed borne out and discussed in
\cref{sec:Evaluation}.

We represent the coverage data for a corpus as a matrix: each row
corresponds to one seed, and each column to a possible edge between
basic blocks in the target.  Such a matrix $A$ has $A_{ij} = 1$ if
seed $i$ causes the target to traverse edge $j$, and is zero
otherwise.

Given this, the objective is to find $\mathit{minset}(A)$: the
smallest weighted set of seeds that covers all of the columns (edges)
in matrix $A$ that have at least one non-zero value.  (A column in $A$
consisting of all zeroes represents an edge never taken by any of the
seeds.)

The unweighted version of the problem (MSCP as defined in
\cref{sec:FormalCorpusDistillation}) simply finds the smallest set of
rows (i.e., seeds) that spans all of the columns.  In the following
presentation we generally do not distinguish between the weighted and
unweighted formulations except where the distinction is important to
the computation.

\subsection{Solution}

Our \tool algorithm applies dynamic programming to take a large
coverage matrix and recursively transform it through row and column
eliminations into successively smaller matrices while accumulating a
minimum cover set \coverset.  As discussed in
\cref{sec:FormalCorpusDistillation}, \coverset is the minimum
collection of seeds that still spans all the observed edges in the
target when dynamically traced.  \coverset becomes our
\emph{distilled} corpus that we perform fuzzing campaigns with.

The following sections describe the matrix operations that produce
\coverset.  This culminates with the presentation of the \tool
algorithm in \cref{sec:tool-algo}.

\subsubsection{Matrix Operations}\label{sec:matrix-ops}
The corpus coverage matrix $A$ is typically large and sparse.  For
example, the number of seeds $N$ in the corpus can be of the order of
$10^5$ files, while the number of observed edges is of the order of
$10^6$.  Combined, the coverage matrix is of the order of $10^{11}$
elements.

Here we present an intuitive description of our operational
primitives, which allow us to transform the large original problem
into smaller over-lapping sub-problems.
%%
% \footnote{A more formal presentation of these operations appears in
%   \cref{sec:Theory-Appendix}.}
%%
We proceed with the working example in
\cref{fig:WorkingExampleMain}.  In this example, rows $s_i$ represent
seeds and columns $e_i$ represent all possible edges.

\input{approach-figs}

\paragraph{Singularities}\label{singularities}
We define the term \emph{singularity} to describe the situation where
a column or row sum is \emph{zero}.  Row sum singularities represent
seeds that do not cover any code when parsed by the target.  These
seeds are rare in practice and can simply be ignored.  In contrast,
column singularities are very common.  Column singularities are an
artifact of tracing tools that identified \emph{all} edges in the
target.

Consider \cref{fig:SingularityMain} from the working example.  Column
$e_6$ (shown in green) is a singular column.  We can eliminate this
column to produce a smaller matrix $A'$ whose minimum cover set
\coverset is the same as the original matrix $A$.

\paragraph{Exotic rows}
An \emph{exotic row} is a row in $A$ that is the only row covering a
particular edge.  For example in \cref{fig:ExoticMain} the row $s_1$
(shown in blue) is exotic because it is the only row that covers
column $e_3$.  All seeds associated with exotic rows are by definition
a part of the final solution and will be included in the distilled
corpus.

\paragraph{Dominant rows}
Row dominance captures the intuitive idea that some rows in $A$ may be
a subset of a single row.  The larger row \emph{dominates} the smaller
\emph{submissive} row which is a subset of the \emph{dominator}.  A
dominant row may in turn be dominated.  Intuitively, all submissive
rows can be deleted from the coverage matrix $A$.  However, this
operation is row weight sensitive.  If the submissive row has a larger
row weight than the dominator then it can be deleted, else it is left
alone because it may ultimately lead to a smaller weighted corpus.

Continuing with the (unweighted) working example in
\cref{fig:RowDominanceMain} we identify row $s_5$ as a dominant row
(shown in red) since it dominates rows $\{s_2,s_3,s_4\}$ (shown in
yellow).  The three submissive rows can be deleted from the matrix.

\paragraph{Dominant columns}
Column dominance is a similar idea to row dominance.  Here, some
columns in $A$ may be a subset of a single column.  However, in this
operation the dominant column is deleted and the submissive columns
are left alone.  This is because any final solution by definition will
contain seeds that cover the submissive columns and by implication
they will also cover the dominant column.  The dominant column is
redundant and can be safely removed.

Continuing with the working example in \cref{fig:ColumnDominanceMain},
we identify column $e_5$ (shown in red) as a dominant column since it
dominates columns $\{e_1,e_3,e_4\}$.  $e_2$ is not dominated by $e_5$
because of $s_2$.

\paragraph{Contained columns}
When choosing row $s_i$ to add to our solution we can eliminate all
the columns that $s_i$ covers.  We call this operation \emph{contained
  column eliminations}.  The columns can be safely deleted because
they will be covered by the seed associated with row $s_i$.
%%This is a very powerful technique for reducing the dimensionality of
%%the problem.

\paragraph{Heuristic rows}
The row and column eliminations described previously have been
\emph{optimal} in the sense that they guarantee an optimal solution
for a smaller transformed matrix can be used to construct an optimal
solution for the larger matrix.  However, there are times when all
optimal operations are exhausted and the algorithm must make a
\emph{heuristic choice} to select a row to add to \coverset.
Intuitively, a good heuristic is to select the row with the largest
$\mathit{rowsum}$, since this will trigger a large \emph{contained
  columns elimination}.  In the weighted case, we choose the row with
the largest $\mathit{rowsum}/\mathit{rowweight}$.  The expectation is
that optimal operations can be resumed on the smaller matrix.

\subsubsection{The \tool Algorithm}\label{sec:tool-algo}

We now present the \tool algorithm.
%%\tool uses dynamic programming to accumulate a near-optimal \coverset.
%%This is achieved by successively applying the matrix operations described in \cref{sec:matrix-ops} until they result in the null matrix.
Given our matrix operators (\cref{sec:matrix-ops}), we use a dynamic programming formulation of the problem to compute a sequence of operations to construct \coverset.
The strategy is to apply these operators until the final operation results in the Null matrix, at which point no further operations are possible.

\paragraph*{Dynamic programming formulation}\label{DP}

%%Given our matrix operators, we use a dynamic programming formulation of the problem to compute a near-optimal sequence of operations to construct \coverset.
%%This allows us to give a compact inductive presentation of our algorithm.
Dynamic programming analysis begins with identifying
%
\begin{myinlinelist}
  \item the cost function of a \emph{state} in terms of a transition cost, and
  \item the subsequent cost of the new, smaller state.
\end{myinlinelist}
%
Here, we define this state to be the coverage matrix $A$ and the cost to be the measure of divergence from an optimal \coverset.
%%If the cost is non-zero then this cost measures the divergence from an optimal \coverset.
This cost is computed as the cost of any of the matrix operations performed on $A$, \emph{plus} the cost of the subsequent state $A'$.

What are the costs for each matrix operation?  Recall that our
objective is to find an optimal \coverset if possible, or measure
divergence from optimality when necessary.  Thus, any optimal row or
column elimination has zero cost because they contribute to an optimal
\coverset.  Optimal reductions occur when
$\mathit{minset}(A) = \mathit{minset}(A')\, \bigcup\, \textit{ExoticRow}$.  We
specify these reductions to have a zero cost \textit{iff} the matrix
size is reduced (i.e., $A \neq A'$); otherwise they have an infinite
cost.  For example, removing column singularities and selecting exotic
rows are all optimal operations and incur no cost providing they
reduce the size of the matrix $A'$.  In contrast, heuristic row
reductions cannot be guaranteed to be an optimal reduction.
Therefore, we define the dynamic programming cost of this operation to
be: \begin{myinlinelist}\item \emph{one} for unweighted set cover;
  or \item $\mathit{rowweight}$ for weighted set
  cover\end{myinlinelist}.

\paragraph{\tool pseudocode}
We present pseudocode for \tool in \cref{alg:Moonshine}.  The ordering
of the five basic matrix operations reflects the relative importance
of those operations in either dimensional reduction, selecting
necessary rows, or computational complexity.
%%Given that matrix operation costs are zero apart from heuristic choice, this formulation of the algorithm is a correct encoding of the Bellman Equation outlined in \cref{DP}.
Observe that the heuristic row choice (i.e., the non-optimal
operation) is the last-resort option.

\begin{algorithm}[h]
  \footnotesize
\begin{algorithmic} % [1]
\Function{\tool}{$A$, $X$}
    \If {$\mathit{isEmpty}(A)$}
		\State \Return $X$
	\EndIf
    \State \Comment {Singularities}
    \State $\mathit{Cols} \leftarrow \mathit{Singularities}(A)$
    \If {$\mathit{Cols} \neq \emptyset$}
        \State $A' \leftarrow \mathit{RemoveRowsCols}(A, \emptyset, \mathit{Cols})$
		\State \Return \Call{\tool}{$A'$, $X$}
	\EndIf
    \State \Comment {Exotic rows}
    \State $\mathit{Rows} \leftarrow \mathit{Exotic}(A)$
    \If { $\mathit{Rows} \neq \emptyset$}
        \State $\mathit{Cols} \leftarrow \mathit{ContainedCols}(A, \mathit{Rows})$
        \State $A' \leftarrow \mathit{RemoveRowsCols}(A, \mathit{Rows}, \mathit{Cols})$
		\State $ X' \leftarrow X \bigcup Rows$
		\State \Return \Call{\tool}{$A'$, $X'$}
	\EndIf
    \State \Comment {Dominant rows}
    \State $\mathit{Rows} \leftarrow \mathit{DominantRows}(A)$
    \If { $\mathit{Rows} \neq \emptyset$}
        \State $A' \leftarrow \mathit{RemoveRowsCols}(A, \mathit{Rows}, \emptyset)$
		\State \Return \Call{\tool}{$A', X$}
	\EndIf
    \State \Comment {Dominant columns}
    \State $\mathit{Cols} \leftarrow \mathit{DominantCols}(A)$
    \If { $\mathit{Cols} \neq \emptyset$}
        \State $A' \leftarrow \mathit{RemoveRowsCols}(A, \emptyset, \mathit{Cols})$
		\State \Return \Call{\tool}{$A'$, $X$}
	\EndIf
    \State \Comment {Heuristic rows}
    \State $\mathit{Rows} \leftarrow \mathit{Heuristic}(A)$
    \State $\mathit{Cols} \leftarrow \mathit{ContainedCols}(A, \mathit{Rows})$
    \State $A' \leftarrow \mathit{RemoveRowsCols}(A, \mathit{Rows}, \mathit{Cols})$
    \State $X'  \leftarrow X \bigcup \mathit{Rows}$
	\State \Return \Call{\tool}{$A'$, $X'$}
\EndFunction
\State \Comment{Entry point}
\State $\mathit{Solution} \leftarrow$ \Call{\tool}{$A$, $\emptyset$}
\end{algorithmic}
\caption{\tool}
\label{alg:Moonshine}
\end{algorithm}


\subsection{Motivating Weighted Corpus Distillations}

Industrial-scale fuzzing involves a large number of worker processes campaigning
on a given target.  For example, Google reports that ClusterFuzz runs \num{5000}
fuzzers on over \num{25000} cores, churning \emph{4 trillion} test-cases a
week~\cite{Google:2019:ClusterFuzzBlackHat, Google:2019:ClusterFuzzBlog,
OSSFuzz:2016}.  This places a large I/O burden on the fuzzing infrastructure, as
test-cases must be fetched/loaded from the global corpus, saved to the (local)
fuzzing queue (when new code is discovered), and synchronized with the global
corpus (so that new coverage can be shared with the other worker
processes).\footnote{Not all fuzzers synchronize with an explicit global corpus.
Instead, they may synchronize with the other worker processes' queues directly.}

\citet{Xu:2017} demonstrate the impact that file system contention has
on industrial-scale fuzzing: despite fuzzing being
embarrassingly-parallel, the number of test-case executions saturates
at 15 cores, degrades at 30 cores, and collapses at 120 cores.  This
collapse is due to overhead from opening/closing test-cases ($2\times$
slowdown) and queue syncing between workers (a further $2\times$
overhead).  In our experiments, we found that syncing accounted for
\SI{63.78}{\percent} of the operations that wrote to the fuzzing queue
(and hence to the file system).  As noted by \citet{Xu:2017}, this
time spent syncing (hence re-executing test-cases from previous worker
processes) is time diverted from mutating inputs and expanding
coverage.  Therefore, a weighted corpus distillation, minimizing the
total collective byte size of the fuzzing corpus, alleviates the I/O
demand on the storage system.  Given this, practical fuzzing would
seem to benefit most from using file-size weighted distillations
compared to unweighted.
%Empirically, this benefit is indeed borne out.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "moonlight"
%%% End:

